AutoPlan: Automatic Planning of Interactive Decision-Making Tasks With Large Language Models

Recent large language models (LLMs) are promising for making decisions in grounded environments. However, LLMs frequently fail in complex decision-making tasks due to the misalignment between the pre-trained knowledge in LLMs and the actual rules in the environment. Existing methods require either costly gradient computation or lengthy in-context demonstrations. In this paper, we propose AutoPlan, an approach to guide LLM-based agents to accomplish interactive decision-making tasks. AutoPlan augments the LLM prompt with a task-solving plan and optimizes it through iterative experience collection and reflection. Our experiments show that AutoPlan, though using no in-context demonstrations, achieves success rates on par with the baselines using human-written demonstrations on ALFWorld and even outperforms them by 8% on HotpotQA. The code is available at https://github.com/owaski/AutoPlan.

==> table/alfworld.tex <==
\begin{table*}[h!]
    \centering
    \begin{tabular}{l|cccccc}\toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{c}{\textbf{ALFWorld Success Rate (\%)}}\\
        & \textit{Pick} & \textit{Light} & \textit{Clean} & \textit{Heat} & \textit{Cool} & \textit{Pick Two} \\
        \midrule 
        ReAct-Direct & 92\% & 94\% & 87\% & 35\% & 71\% & 59\% \\
        ReAct-ICL  & 83\% & 83\% & 61\% & 61\% & \textbf{86\%} & 35\% \\
        \method  & \textbf{96\%} & \textbf{100\%} & \textbf{94\%} & \textbf{96\%} & 81\% & \textbf{59\%} \\
        \midrule
        Supervised Baseline & 
        \bottomrule
    \end{tabular}
    \caption{Success rate of methods on HotpotQA with a simple wikipedia API and ALFWorld.}
    \label{tab:main}
\end{table*}
